Normalization for planar string diagrams and a quadratic equivalence algorithm

In the graphical calculus of planar string diagrams, equality is generated by exchange moves, which swap the heights of adjacent vertices. We show that left- and right-handed exchanges each give strongly normalizing rewrite strategies for connected string diagrams. We use this result to give a linear-time solution to the equivalence problem in the connected case, and a quadratic solution in the general case. We also give a stronger proof of the Joyal-Street coherence theorem, settling Selinger's conjecture on recumbent isotopy.

==> figures/connected-via-boundary-lics.tex <==
\begin{figure}[b]
  \centering
  \begin{subfigure}{0.23\textwidth}
    \centering
    \begin{tikzpicture}[scale=0.32]
      \startdiagram{3}
      \drawinitialstrands{3}
      \diagslice{1}{0}{1}
      \diagslice{2}{1}{0}
      \diagslice{2}{0}{1}
      \diagslice{0}{1}{0}
      \diagslice{0}{2}{1}
      \finishdiagram
    \end{tikzpicture}
    \caption{The original diagram $D$}
    \label{fig:connected-via-boundary-a}
  \end{subfigure}
    \begin{subfigure}{0.23\textwidth}
      \centering
      \vspace{-.5cm}
    \begin{tikzpicture}[scale=0.22]
      \startdiagram{1}
      \reddiagslice{0}{0}{4}
      \diagslice{2}{0}{1}
      \diagslice{3}{1}{0}
      \diagslice{3}{0}{1}
      \diagslice{1}{1}{0}
      \diagslice{1}{2}{1}
      \reddiagslice{0}{3}{0}
      \storeedgecolor{0}{red}
      \storeedgecolor{3}{red}
      \finishdiagram
      \node[rnode] at (v0) {};
      \node[rnode] at (v6) {};
      \node[node distance=.3cm,above of=v0,red] {$t$};
      \node[node distance=.3cm,below of=v6,red] {$b$};
    \end{tikzpicture}
    \caption{The transformed diagram $D'$}
  \end{subfigure}
  \caption{Adding nodes on the boundaries to make a diagram connected} \label{fig:connected-via-boundary}
\end{figure}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: ../lics
%%% End:


==> figures/spirals.tex <==
\begin{figure}[H]
  \centering
  \newcommand\drawspiral[1]{%
    \begin{scope}[yscale=0.5]
      \node[bnode] at (0,-1) (p) {};
      \pgfmathsetmacro\bnd{#1-1}
      \foreach \y in {1,...,\bnd} {
        \ifodd\y
        \def\pos{\y}
        \else
        \def\pos{-\y-1}
        \fi
        \draw (p) edge[bend right] (0,\pos);
        \node[bnode] at (0,\pos) (p) {};
      }
    \end{scope}
  }
  \begin{tikzpicture}[scale=0.5]
    \begin{scope}[xshift=1cm]
    \node[bnode] at (0,-1) (a) {};
    \node[bnode] at (0,0) (b) {};
    \draw (a) -- (b);
    \node at (-1.5,-.5) {$S_2 = $};
    \end{scope}
    
    \foreach \n in {3,...,5} {%
      \pgfmathsetmacro\sft{-11+5.5*\n}
      \begin{scope}[xshift=\sft cm]
        \node at (-2.5,-.5) {$S_\n = $};
        \drawspiral{\n}
      \end{scope}}
    \begin{scope}[xshift=21cm,xscale=-1]
      \drawspiral{5}
      \node at (2.1,-.5) {$\Rarrowstar$};
    \end{scope}
  \end{tikzpicture}
\end{figure}
  
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../project"
%%% End:

